QUASAR: QUality and Aesthetics Scoring with Advanced Representations

This paper introduces a new data-driven, non-parametric method for image quality and aesthetics assessment, surpassing existing approaches and requiring no prompt engineering or fine-tuning. We eliminate the need for expressive textual embeddings by proposing efficient image anchors in the data. Through extensive evaluations of 7 state-of-the-art self-supervised models, our method demonstrates superior performance and robustness across various datasets and benchmarks. Notably, it achieves high agreement with human assessments even with limited data and shows high robustness to the nature of data and their pre-processing pipeline. Our contributions offer a streamlined solution for assessment of images while providing insights into the perception of visual information.

==> ECCV/chapters/11_references.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})



@misc{Authors14,
 author = {FirstName LastName},
 title = {The frobnicatable foo filter},
 note = {Face and Gesture submission ID 324. Supplied as supplemental material {\tt fg324.pdf}},
 year = 2014
}

@misc{Authors14b,
 author = {FirstName LastName},
 title = {Frobnication tutorial},
 note = {Supplied as supplemental material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {FirstName Alpher},
title = {Frobnication},
journal = PAMI,
volume = 12,
number = 1,
pages = {234--778},
year = 2002
}

@article{Alpher03,
author = {FirstName Alpher and  FirstName Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13,
number = 1,
pages = {234--778},
year = 2003
}

@article{Alpher04,
author = {FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14,
number = 1,
pages = {234--778},
year = 2004
}

@inproceedings{Alpher05,
author = {FirstName Alpher and FirstName Gamow},
title = {Can a computer frobnicate?},
booktitle = CVPR,
pages = {234--778},
year = 2005
}

% PIPAL dataset
@inproceedings{jinjin2020pipal,
  title={Pipal: a large-scale image quality assessment dataset for perceptual image restoration},
  author={Jinjin, Gu and Haoming, Cai and Haoyu, Chen and Xiaoxing, Ye and Ren, Jimmy S and Chao, Dong},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part XI 16},
  pages={633--651},
  year={2020},
  organization={Springer}
}


@inproceedings{Lin2019kadid10k,
title={KADID-10k: A Large-scale Artificially 
Distorted IQA Database},
author={Lin, Hanhe and Hosu, Vlad and Saupe, Dietmar},
booktitle={2019 Tenth International Conference on 
Quality of Multimedia Experience (QoMEX)},
pages={1--3},
year={2019},
organization={IEEE}}


@article{ponomarenko2015image,
  title={Image database TID2013: Peculiarities, results and perspectives},
  author={Ponomarenko, Nikolay and Jin, Lina and Ieremeiev, Oleg and Lukin, Vladimir and Egiazarian, Karen and Astola, Jaakko and Vozel, Benoit and Chehdi, Kacem and Carli, Marco and Battisti, Federica and others},
  journal={Signal processing: Image communication},
  volume={30},
  pages={57--77},
  year={2015},
  publisher={Elsevier}
}


@article{hosu2020koniq10k,
author={V. {Hosu} and H. {Lin} and T. {Sziranyi} and D. 
{Saupe}},
journal={IEEE Transactions on Image Processing},
title={KonIQ-10k: An Ecologically Valid Database for Deep 
Learning of Blind Image Quality Assessment},
year={2020},
volume={29},
pages={4041-4056}}

@inproceedings{murray2012ava,
  title={AVA: A large-scale database for aesthetic visual analysis},
  author={Murray, Naila and Marchesotti, Luca and Perronnin, Florent},
  booktitle={2012 IEEE conference on computer vision and pattern recognition},
  pages={2408--2415},
  year={2012},
  organization={IEEE}
}

@article{ghadiyaram2015massive,
  title={Massive online crowdsourced study of subjective and objective picture quality},
  author={Ghadiyaram, Deepti and Bovik, Alan C},
  journal={IEEE Transactions on Image Processing},
  volume={25},
  number={1},
  pages={372--387},
  year={2015},
  publisher={IEEE}
}

% SPAQ dataset
@inproceedings{fang2020perceptual,
  title={Perceptual quality assessment of smartphone photography},
  author={Fang, Yuming and Zhu, Hanwei and Zeng, Yan and Ma, Kede and Wang, Zhou},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3677--3686},
  year={2020}
}

% TAD66k dataset
@inproceedings{he2022rethinking,
  title={Rethinking image aesthetics assessment: Models, datasets and benchmarks},
  author={He, Shuai and Zhang, Yongchang and Xie, Rui and Jiang, Dongxiang and Ming, Anlong},
  booktitle={Proceedings of the Thirty-First International Joint Conference on Artificial Intelligence, IJCAI-22},
  pages={942--948},
  year={2022}
}

% AADB dataset and metric
@inproceedings{kong2016photo,
  title={Photo aesthetics ranking network with attributes and content adaptation},
  author={Kong, Shu and Shen, Xiaohui and Lin, Zhe and Mech, Radomir and Fowlkes, Charless},
  booktitle={Computer Vision--ECCV 2016: 14th European Conference, Amsterdam, The Netherlands, October 11--14, 2016, Proceedings, Part I 14},
  pages={662--679},
  year={2016},
  organization={Springer}
}

% CLIP-IQA
@inproceedings{wang2023exploring,
  title={Exploring clip for assessing the look and feel of images},
  author={Wang, Jianyi and Chan, Kelvin CK and Loy, Chen Change},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={37},
  number={2},
  pages={2555--2563},
  year={2023}
}

% CLIP
@inproceedings{radford2021learning,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  booktitle={International conference on machine learning},
  pages={8748--8763},
  year={2021},
  organization={PMLR}
}

% ALIGN
@inproceedings{jia2021align,
  title={Scaling up visual and vision-language representation learning with noisy text supervision},
  author={Jia, Chao and Yang, Yinfei and Xia, Ye and Chen, Yi-Ting and Parekh, Zarana and Pham, Hieu and Le, Quoc and Sung, Yun-Hsuan and Li, Zhen and Duerig, Tom},
  booktitle={International conference on machine learning},
  pages={4904--4916},
  year={2021},
  organization={PMLR}
}


% BLIP
@inproceedings{li2022blip,
  title={Blip: Bootstrapping language-image pre-training for unified vision-language understanding and generation},
  author={Li, Junnan and Li, Dongxu and Xiong, Caiming and Hoi, Steven},
  booktitle={International Conference on Machine Learning},
  pages={12888--12900},
  year={2022},
  organization={PMLR}
}

% BLIP-2
@article{li2023blip2,
  title={Blip-2: Bootstrapping language-image pre-training with frozen image encoders and large language models},
  author={Li, Junnan and Li, Dongxu and Savarese, Silvio and Hoi, Steven},
  journal={arXiv preprint arXiv:2301.12597},
  year={2023}
}



% DINO
@inproceedings{caron2021emerging,
  title={Emerging properties in self-supervised vision transformers},
  author={Caron, Mathilde and Touvron, Hugo and Misra, Ishan and J{\'e}gou, Herv{\'e} and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={9650--9660},
  year={2021}
}

% DINOv2
@article{oquab2023dinov2,
  title={Dinov2: Learning robust visual features without supervision},
  author={Oquab, Maxime and Darcet, Timoth{\'e}e and Moutakanni, Th{\'e}o and Vo, Huy and Szafraniec, Marc and Khalidov, Vasil and Fernandez, Pierre and Haziza, Daniel and Massa, Francisco and El-Nouby, Alaaeldin and others},
  journal={arXiv preprint arXiv:2304.07193},
  year={2023}
}


% CoCA
@article{yu2022coca,
  title={Coca: Contrastive captioners are image-text foundation models},
  author={Yu, Jiahui and Wang, Zirui and Vasudevan, Vijay and Yeung, Legg and Seyedhosseini, Mojtaba and Wu, Yonghui},
  journal={arXiv preprint arXiv:2205.01917},
  year={2022}
}

% ViT
@article{dosovitskiy2020image,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}

% ResNet, RN
@inproceedings{jian2016deep,
  title={Deep residual learning for image recognition},
  author={Jian, S and Kaiming, H and Shaoqing, R and Xiangyu, Z},
  booktitle={IEEE Conference on Computer Vision \& Pattern Recognition},
  pages={770--778},
  year={2016}
}

% ImageNet dataset
@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},

  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
} 

% k-means clustering
@article{lloyd1982least,
  title={Least squares quantization in PCM},
  author={Lloyd, Stuart},
  journal={IEEE transactions on information theory},
  volume={28},
  number={2},
  pages={129--137},
  year={1982},
  publisher={IEEE}
}

@ARTICLE{our_iqa_for_mri_paper_r,

  author={Kastryulin and others},

  journal={IEEE Access}, 

  year={2023},

  volume={11},

  number={},

  pages={14154}
}

@ARTICLE{our_iqa_for_mri_paper,

  author={Kastryulin, Sergey and Zakirov, Jamil and Pezzotti, Nicola and Dylov, Dmitry V.},

  journal={IEEE Access}, 

  title={Image Quality Assessment for Magnetic Resonance Imaging}, 

  year={2023},

  volume={11},

  number={},

  pages={14154-14168},

  keywords={Measurement;Magnetic resonance imaging;Image quality;Biomedical imaging;Signal to noise ratio;Deep learning;Distortion;Image quality;deep learning;metrics;reconstruction quality;MRI}
}


% OpenCLIP code
@software{ilharco_gabriel_2021_5143773,
  author       = {Ilharco, Gabriel and
                  Wortsman, Mitchell and
                  Wightman, Ross and
                  Gordon, Cade and
                  Carlini, Nicholas and
                  Taori, Rohan and
                  Dave, Achal and
                  Shankar, Vaishaal and
                  Namkoong, Hongseok and
                  Miller, John and
                  Hajishirzi, Hannaneh and
                  Farhadi, Ali and
                  Schmidt, Ludwig},
  title        = {OpenCLIP},
  month        = jul,
  year         = 2021,
  note         = {If you use this software, please cite it as below.},
  publisher    = {Zenodo},
  version      = {0.1},
  doi          = {10.5281/zenodo.5143773},
  url          = {https://doi.org/10.5281/zenodo.5143773}
}

% OpenCLIP paper
@inproceedings{cherti2023reproducible,
  title={Reproducible scaling laws for contrastive language-image learning},
  author={Cherti, Mehdi and Beaumont, Romain and Wightman, Ross and Wortsman, Mitchell and Ilharco, Gabriel and Gordon, Cade and Schuhmann, Christoph and Schmidt, Ludwig and Jitsev, Jenia},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2818--2829},
  year={2023}
}

% piq paper
@misc{kastryulin2022piq,
  title = {PyTorch Image Quality: Metrics for Image Quality Assessment},
  url = {https://arxiv.org/abs/2208.14818},
  author = {Kastryulin, Sergey and Zakirov, Jamil and Prokopenko, Denis and Dylov, Dmitry V.},
  doi = {10.48550/ARXIV.2208.14818},
  publisher = {arXiv},
  year = {2022}
}

% piq code
@misc{piq,
  title={{PyTorch Image Quality}: Metrics and Measure for Image Quality Assessment},
  url={https://github.com/photosynthesis-team/piq},
  note={Open-source software available at https://github.com/photosynthesis-team/piq},
  author={Sergey Kastryulin and Dzhamil Zakirov and Denis Prokopenko},
  year={2019}
}

% BIQI metric
@article{moorthy2010two,
  title={A two-step framework for constructing blind image quality indices},
  author={Moorthy, Anush Krishna and Bovik, Alan Conrad},
  journal={IEEE Signal processing letters},
  volume={17},
  number={5},
  pages={513--516},
  year={2010},
  publisher={IEEE}
}

% BLIINDS-II metric
@article{saad2012blind,
  title={Blind image quality assessment: A natural scene statistics approach in the DCT domain},
  author={Saad, Michele A and Bovik, Alan C and Charrier, Christophe},
  journal={IEEE transactions on Image Processing},
  volume={21},
  number={8},
  pages={3339--3352},
  year={2012},
  publisher={IEEE}
}

% BRISQUE metric
@article{mittal2012no,
  title={No-reference image quality assessment in the spatial domain},
  author={Mittal, Anish and Moorthy, Anush Krishna and Bovik, Alan Conrad},
  journal={IEEE Transactions on image processing},
  volume={21},
  number={12},
  pages={4695--4708},
  year={2012},
  publisher={IEEE}
}

% NIQE metric
@article{mittal2012making,
  title={Making a “completely blind” image quality analyzer},
  author={Mittal, Anish and Soundararajan, Rajiv and Bovik, Alan C},
  journal={IEEE Signal processing letters},
  volume={20},
  number={3},
  pages={209--212},
  year={2012},
  publisher={IEEE}
}

% RAPID metric
@inproceedings{lu2014rapid,
  title={Rapid: Rating pictorial aesthetics using deep learning},
  author={Lu, Xin and Lin, Zhe and Jin, Hailin and Yang, Jianchao and Wang, James Z},
  booktitle={Proceedings of the 22nd ACM international conference on Multimedia},
  pages={457--466},
  year={2014}
}

A-lamp metric
@inproceedings{ma2017lamp,
  title={A-lamp: Adaptive layout-aware multi-patch deep convolutional neural network for photo aesthetic assessment},
  author={Ma, Shuang and Liu, Jing and Wen Chen, Chang},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4535--4544},
  year={2017}
}

% NIMA metric
@article{talebi2018nima,
  title={NIMA: Neural image assessment},
  author={Talebi, Hossein and Milanfar, Peyman},
  journal={IEEE transactions on image processing},
  volume={27},
  number={8},
  pages={3998--4011},
  year={2018},
  publisher={IEEE}
}


@article{antsiferova2023comparing,
  title={Comparing the robustness of modern no-reference image-and video-quality metrics to adversarial attacks},
  author={Antsiferova, Anastasia and Abud, Khaled and Gushchin, Aleksandr and Lavrushkin, Sergey and Shumitskaya, Ekaterina and Velikanov, Maksim and Vatolin, Dmitriy},
  journal={arXiv preprint arXiv:2310.06958},
  year={2023}
}


@article{kettunen2019lpips,
  title={E-lpips: robust perceptual image similarity via random transformation ensembles},
  author={Kettunen, Markus and H{\"a}rk{\"o}nen, Erik and Lehtinen, Jaakko},
  journal={arXiv preprint arXiv:1906.03973},
  year={2019}
}


@article{shumitskaya2022universal,
  title={Universal perturbation attack on differentiable no-reference image-and video-quality metrics},
  author={Shumitskaya, Ekaterina and Antsiferova, Anastasia and Vatolin, Dmitriy},
  journal={arXiv preprint arXiv:2211.00366},
  year={2022}
}

@inproceedings{sheng2023aesclip,
  title={AesCLIP: Multi-Attribute Contrastive Learning for Image Aesthetics Assessment},
  author={Sheng, Xiangfei and Li, Leida and Chen, Pengfei and Wu, Jinjian and Dong, Weisheng and Yang, Yuzhe and Xu, Liwu and Li, Yaqian and Shi, Guangming},
  booktitle={Proceedings of the 31st ACM International Conference on Multimedia},
  pages={1117--1126},
  year={2023}
}

% CLIP object detection
@article{lin2023gridclip,
  title={GridCLIP: One-Stage Object Detection by Grid-Level CLIP Representation Learning},
  author={Lin, Jiayi and Gong, Shaogang},
  journal={arXiv preprint arXiv:2303.09252},
  year={2023}
}

% CLIP semantic segmentation
@inproceedings{zhou2023zegclip,
  title={Zegclip: Towards adapting clip for zero-shot semantic segmentation},
  author={Zhou, Ziqin and Lei, Yinjie and Zhang, Bowen and Liu, Lingqiao and Liu, Yifan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={11175--11185},
  year={2023}
}

% Stable Diffusion
@misc{rombach2021highresolution,
      title={High-Resolution Image Synthesis with Latent Diffusion Models}, 
      author={Robin Rombach and Andreas Blattmann and Dominik Lorenz and Patrick Esser and Björn Ommer},
      year={2021},
      eprint={2112.10752},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

% unCLIP
@article{ramesh2022unclip,
  title={Hierarchical text-conditional image generation with clip latents},
  author={Ramesh, Aditya and Dhariwal, Prafulla and Nichol, Alex and Chu, Casey and Chen, Mark},
  journal={arXiv preprint arXiv:2204.06125},
  volume={1},
  number={2},
  pages={3},
  year={2022}
}

@phdthesis{wang2006modern,
  title={Modern image quality assessment},
  author={Wang, Zhou and Bovik, Alan Conrad},
  year={2006},
  school={Springer}
}

@inproceedings{sheikh2005visual,
  title={A visual information fidelity approach to video quality assessment},
  author={Sheikh, Hamid R and Bovik, Alan C},
  booktitle={The first international workshop on video processing and quality metrics for consumer electronics},
  volume={7},
  number={2},
  pages={2117--2128},
  year={2005},
  organization={sn}
}


@article{zhang2011fsim,
  title={FSIM: A feature similarity index for image quality assessment},
  author={Zhang, Lin and Zhang, Lei and Mou, Xuanqin and Zhang, David},
  journal={IEEE transactions on Image Processing},
  volume={20},
  number={8},
  pages={2378--2386},
  year={2011},
  publisher={IEEE}
}


@inproceedings{prashnani2018pieapp,
  title={Pieapp: Perceptual image-error assessment through pairwise preference},
  author={Prashnani, Ekta and Cai, Hong and Mostofi, Yasamin and Sen, Pradeep},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1808--1817},
  year={2018}
}


@inproceedings{cheon2021perceptual,
  title={Perceptual image quality assessment with transformers},
  author={Cheon, Manri and Yoon, Sung-Jun and Kang, Byungyeon and Lee, Junwoo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={433--442},
  year={2021}
}


@inproceedings{lao2022attentions,
  title={Attentions help cnns see better: Attention-based hybrid image quality assessment network},
  author={Lao, Shanshan and Gong, Yuan and Shi, Shuwei and Yang, Sidi and Wu, Tianhe and Wang, Jiahao and Xia, Weihao and Yang, Yujiu},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={1140--1149},
  year={2022}
}

% Large study on IQA
@article{sara2019iqa_survey,
  title={Image quality assessment through FSIM, SSIM, MSE and PSNR—a comparative study},
  author={Sara, Umme and Akter, Morium and Uddin, Mohammad Shorif},
  journal={Journal of Computer and Communications},
  volume={7},
  number={3},
  pages={8--18},
  year={2019},
  publisher={Scientific Research Publishing}
}

@inproceedings{prashnani2018pieapp,
  title={Pieapp: Perceptual image-error assessment through pairwise preference},
  author={Prashnani, Ekta and Cai, Hong and Mostofi, Yasamin and Sen, Pradeep},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1808--1817},
  year={2018}
}

==> ECCV/figs/aestetics-cv.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/aestetics_srcc_cv.pdf}
    \caption{Aesthetics SRCC.}
    \label{fig:a-cv}
\end{figure}

https://www.overleaf.com/project/651e84735ecc94d2f1d6f401

==> ECCV/figs/aesthetics-clusters.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/aesthetics_srcc_clusters.pdf}
    \caption{Aesthetics SRCC for clusters.}
    \label{fig:a-clusters}
\end{figure}



==> ECCV/figs/aesthetics-ratio-all.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/aesthetics_ratio_all.pdf}
    \caption{Aesthetics SRCC. Prompt ratio.}
    \label{fig:a-ratio-all}
\end{figure}



==> ECCV/figs/experiments_1_best.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[]{figs/source/experiments_1_best.pdf}
    \caption{Aggregating the best performance of QUASAR and CLIP-IQA metrics on 5 IQA and 2 IAA benchmarks. 
    Note the large performance gain on widely used TID2014, KADID10k, and the most challenging TAD66k datasets.}
    \label{fig:best}
\end{figure}



==> ECCV/figs/experiments_3a_random_ratios.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics{figs/source/experiments_3a_random_ratios.pdf}
    \caption{Different ratios, random pairs.}
    \label{fig:ratio_random}
\end{figure}



==> ECCV/figs/experiments_3b_linked_ratios.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics{figs/source/experiments_3b_linked_ratios.pdf}
    \caption{Different ratios, linked pairs.}
    \label{fig:ratio_linked}
\end{figure}



==> ECCV/figs/experiments_4_linked_ratios_200.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics{figs/source/experiments_4_linked_200.pdf}
    \caption{Different ratios, linked pairs. limit 200}
    \label{fig:ratio_linked_200}
\end{figure}



==> ECCV/figs/experiments_5_random_vs_linked.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics{figs/source/experiments_5_random_vs_linked.pdf}
    \caption{PIPAL, random reference-distorsion pairs vs linked.}
    \label{fig:random_vs_linked}
\end{figure}


==> ECCV/figs/experiments_6_offset.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/experiments_6_offset.pdf}
    \caption{Offset, CLIP RN50, Full res, AVA anchors.}
    \label{fig:offest_CLIP}
\end{figure}



==> ECCV/figs/experiments_7_clusters_1.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/experiments_7_clusters_1.pdf}
    \caption{Aggregation for CLIP RN50 full res, AVA anchors}
    \label{fig:clusters_1}
\end{figure}



==> ECCV/figs/experiments_8_clusters_2.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/experiments_8_clusters_2.pdf}
    \caption{Clusters, All extractors, AVA anchors.}
    \label{fig:clusters_2}
\end{figure}



==> ECCV/figs/experiments_9_offset_all.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/experiments_9_offset_all.pdf}
    \caption{Offset, All extractors, AVA anchors.}
    \label{fig:offest_all}
\end{figure}



==> ECCV/figs/quality-cv.tex <==
% Use figure* for multi-column figure
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/quality_srcc_cv.pdf}
    \caption{Image quality SRCC.}
    \label{fig:q-cv}
\end{figure*}



==> ECCV/figs/quality-ratio-200.tex <==
% Use figure* for multi-column figure
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/quality_ratio_200.pdf}
    \caption{Image quality SRCC. Prompt ratio limited 200.}
    \label{fig:q-ratio-200}
\end{figure*}



==> ECCV/figs/quality-ratio-all.tex <==
% Use figure* for multi-column figure
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/quality_ratio_all.pdf}
    \caption{Image quality SRCC. Prompt ratio.}
    \label{fig:q-ratio-all}
\end{figure*}



==> ECCV/figs/quality-ration-randomvslinked.tex <==
% Use figure* for multi-column figure
\begin{figure*}[tp]
    \centering
    \includegraphics[width=\linewidth]{figs/source/quality_ratio_randomvslinked_CLIP-ViT-L-14.pdf}
    \caption{Image quality SRCC. Prompt ratio when random or linked pairs.}
    \label{fig:q-ratio-randomvslinked}
\end{figure*}



==> ECCV/figs/rebuttal_umap_ava.tex <==
% Use figure* for multi-column figure
\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{figs/rebuttal/ava_umap_scores_200.pdf}
    \caption{Low-dimensional UMAP visualisation of the 100 high- (green) and 100 low-quality (blue) samples from AVA dataset.}
    \label{fig:rebuttal-ava}
\end{figure}



==> ECCV/tables/metrics.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% new example:
\begin{table}[tb]
  \caption{May remove this one when the table with scores is ready.
  }
  \label{tab:metrics}
  \centering
  \begin{tabular}{@{}lcc@{}}
    \toprule
    Metric & Task & Training Set \\
    \midrule
    BIQI \cite{moorthy2010two} & NR IQA & N/A \\
BLIINDS-II \cite{saad2012blind} & NR IQA & N/A \\
BRISQUE \cite{mittal2012no} & NR IQA & N/A \\
NIQE \cite{mittal2012making} & NR IQA & N/A \\
RAPID \cite{lu2014rapid} & IAA & AVA \cite{murray2012ava} \\
AADB \cite{kong2016photo} & IAA & AADB \cite{kong2016photo} + AVA \cite{murray2012ava} \\
A-lamp \cite{ma2017lamp} & IAA & AVA \cite{murray2012ava} \\
NIMA \cite{talebi2018nima} & IAA & AVA \cite{murray2012ava} \\
CLIP-IQA \cite{wang2023exploring} & Generic & N/A \\
QUASAR (ours) & Generic & N/A \\
\bottomrule
  \end{tabular}
  \vspace{-0.05in}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% old example:


==> ECCV/tables/r_pieapp.tex <==

\begin{table}[tb]
  \caption{Comparison of 4 popular no-reference IQA metrics, CLIP-IQA, and QUASAR on PieAPP test set.
  }
  \label{tab:pieapp-metrics}
  \centering
  \begin{tabular}{@{}ll@{}}
    \hline
    Metric & SRCC  \\
    \hline
    BIQI & $0.243$ \\
BLIINDS-II  &  $0.250$ \\
BRISQUE  & $0.328$ \\
NIQE  & $0.182$ \\
\hline
CLIP-IQA& $ 0.288$\\
QUASAR (ours) & $\textbf{0.375}$
  \end{tabular}
  %\vspace{-0.05in}
\end{table}



